SAIL-VOS 3D: A Synthetic Dataset and Baselines for Object Detection and 3D Mesh Reconstruction from Video Data

Extracting detailed 3D information of objects from video data is an important goal for holistic scene understanding. While recent methods have shown impressive results when reconstructing meshes of objects from a single image, results often remain ambiguous as part of the object is unobserved. Moreover, existing image-based datasets for mesh reconstruction don't permit to study models which integrate temporal information. To alleviate both concerns we present SAIL-VOS 3D: a synthetic video dataset with frame-by-frame mesh annotations which extends SAIL-VOS. We also develop first baselines for reconstruction of 3D meshes from video data via temporal models. We demonstrate efficacy of the proposed baseline on SAIL-VOS 3D and Pix3D, showing that temporal information improves reconstruction quality. Resources and additional information are available at http://sailvos.web.illinois.edu.

==> fig_shapenet2.tex <==


\begin{figure*}[h]
\vspace{-0.3cm}
	\begin{minipage}[t]{\textwidth}
	\setlength{\tabcolsep}{1pt}
    \renewcommand{\arraystretch}{0.95}
        \begin{tabular}{ccccc}
 &
        \includegraphics[align=c, width=0.28\textwidth,height=1.2in]{cvpr2021/Figs/results_pix3d/ours_bed.png} 
&
        \includegraphics[align=c, width=0.28\textwidth,height=1.2in]{cvpr2021/Figs/results_pix3d/bed.png} & 			\includegraphics[align=c, width=0.28\textwidth,height=1.2
        in]{cvpr2021/Figs/results_pix3d/sofa.png}& 			\includegraphics[align=c, height=1.5in]{cvpr2021/Figs/results_pix3d/ours_chair.png}  \\
        \end{tabular}
\end{minipage}
\vspace{-0.3cm}
\captionof{figure}{Visualization of 3D reconstruction from our Video2Mesh method on Pix3D.}
\label{fig:shapenet2}
\vspace{-0.6cm}

\end{figure*}



==> tab_depth.tex <==
\begin{table}[t]
	\centering
	\caption{Performance on SAILVOS-3D using RGB and/or depth as input for 3D prediction head.\label{tab:depth}} %
	\vspace*{-0.15in}
	\resizebox{0.65\linewidth}{!}{%
		\begin{tabular}{@{} lcccccccccccc@{} }
			\toprule
			
			RGB & Depth & $\text{AP}^{\text{box}}$ & $\text{AP}^{\text{mask}}$ & $\text{AP}^{\text{mesh}}$  \\
			\midrule 
			\checkmark&-&\\
			-&\checkmark&\\
			\checkmark&\checkmark&\\
			
			\bottomrule
		\end{tabular}
	}
\end{table}


==> tab_shapenet.tex <==
\begin{table*}[h]
\vspace{-0.2cm}
	\centering
	\caption{Evaluation on Pix3D. \label{tab:pix3d}} %
	\vspace*{-0.15in}
	\resizebox{\linewidth}{!}{%
		\begin{tabular}{@{\extracolsep{3pt}} lcccccccccccccccccc @{} }
			\toprule
			\multirow{2}{*}{\%} & \multicolumn{3}{c}{All} & \multicolumn{9}{c}{Per-category $\text{AP}^{\text{mesh}}$} & \multirow{2}{*}{\#Verts} & \multirow{2}{*}{\# Faces}\\
			\cline{2-4} \cline{5-13} 
			& $\text{AP}^{\text{box}}$ & $\text{AP}^{\text{mask}}$ & $\text{AP}^{\text{mesh}}$ & Chair & Sofa & Table & Bed & Desk & Bkcs & Wrdb & Tool & Misc\\
			\midrule 
			Pixel2Mesh$\dagger$ 
			& 93.5 & 88.4 & 39.9 & 30.9 &  59.1 &  40.2 &  40.5 &  30.2 &  50.8  &  62.4   & 18.2 &  26.7 & 2562 & 5120\\
			MeshR-CNN~\cite{gkioxari2019mesh} 
			& 94.0 & 88.4 & \bf 51.1& \bf 48.2 & \bf 71.7 & \bf 60.9 &  \bf 53.7  & \bf 42.9 & \bf 70.2 & \bf  63.4& 21.6 & \bf 27.8 & 2367 & 4743\\
			Ours 
			& \bf 94.1 & \bf 88.6 & 45.8 & 41.3 & 67.1 & 49.5 & 51.3 & 33.7 &  65.2 & 52.3 & \bf 24.7 & 27.0 &1967 & 4000\\
			\bottomrule
		\end{tabular}
	}
	\vspace{-0.2cm}
\end{table*}

